Temporal Adaptive Fine-Tuning for Code Comprehension

Repository-level code comprehension question answering (QA) supports developer reasoning over functionality and usage distributed across codebases. However, repository-specialized large language models (LLMs) can become misaligned as code evolves. We study this challenge as temporal repository adaptation: acquiring new knowledge, suppressing obsolete, retaining still-valid, and preserving semantically neighboring knowledge. Existing retrieval, fine-tuning, and model-editing methods address only parts of this problem. We propose Temporal Adaptive Fine-Tuning (TAFT), a novel adaptation approach that treats repository transitions as supervision. TAFT derives temporally grounded QA data from repository transitions, pairs newly valid with obsolete knowledge through preference optimization, and replays transition-conditioned retention examples to preserve still-valid knowledge. We evaluate TAFT on an augmented temporal SWE-bench dataset comprising 255,295 QA entries across ten temporal slices, comparing deferred (Baseline), per-slice retrained (Baseline-Batched), and variants with knowledge anchors along four dimensions: updated knowledge, obsolete-answer suppression, retention, and neighbor stability. TAFT consistently outperforms both the deferred and batched baselines, with an average relative improvement of 18% in updated/suppressed knowledge accuracy, doubled retention accuracy, and roughly 1.5 times the neighbor accuracy. With directly supplied knowledge anchors, TAFT-KANT further improves mean updated/suppressed, retention, and neighbor accuracy over TAFT by 3.55%, 8.35%, and 13.00%, respectively. Overall, TAFT demonstrates its effectiveness across all evaluated areas, effectively enabling code comprehension QA alignment with repository evolution.

==> macros.tex <==
\usepackage{xspace}
\usepackage{booktabs}
\usepackage[capitalise]{cleveref}
\usepackage{colortbl}
\usepackage[inline]{enumitem}
\usepackage[acronym]{glossaries}
\usepackage{multirow}
\usepackage{siunitx}
\usepackage{threeparttable}

\Crefname{figure}{Figure}{Figures}


\definecolor{gray20}{gray}{.8}
\definecolor{gray05}{gray}{.95}


\newsavebox{\rqboxbox}

\newenvironment{rqbox}
{%
	\par\vspace{0.2em}\noindent
	\begin{lrbox}{\rqboxbox}%
		\begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}%
			\normalsize
			}
			{%
		\end{minipage}%
	\end{lrbox}%
	\fcolorbox{gray20}{gray05}{\usebox{\rqboxbox}}%
	\par\vspace{0.2em}\noindent
}


\RequirePackage[skins,xparse,breakable]{tcolorbox}
\NewTColorBox{custombox}{o}{
  breakable,
	colback=gray!10,
	colframe=gray!70,
	left=1.5mm,
	right=1.5mm,
	top=0.1mm,
	bottom=0.1mm,
	fonttitle=\bfseries,
	arc=0mm,
	leftrule=1mm,
	rightrule=0mm,
	toprule=0mm,
	bottomrule=0mm,
	notitle,
	before=\par\medskip\noindent,
	IfValueTF={\small#1}{before upper={\small\textbf{#1: } }}{},
}

\newcommand{\rqa}{$RQ_1$}
\newcommand{\rqb}{$RQ_2$}
\newcommand{\rqc}{$RQ_3$}
\newcommand{\rqd}{$RQ_4$}


\graphicspath{{figures/}}


\newcommand{\etal}{\emph{et al.,}\xspace}

\usepackage{url}
\makeatletter
\def\url@leostyle{%
	\@ifundefined{selectfont}{\def\UrlFont{\textsf}}{\def\UrlFont{\small\sffamily}}}
\makeatother
\urlstyle{leo}








\sisetup{group-separator={,}, group-minimum-digits=4, group-digits=integer, retain-explicit-plus, text-series-to-math, text-family-to-math}








